OH-Formation Following Vibrationally Induced Reaction Dynamics of H$_2$COO

The reaction dynamics of H$_2$COO to form linear HCOOH and dioxirane as first steps for OH-elimination is quantitatively investigated. Using a machine learned potential energy surface at the CASPT2/aug-cc-pVTZ level of theory vibrational excitation along the CH-normal mode $\nu_{\rm CH}$ with energies up to 40.0 kcal/mol ($\sim 5 \nu_{\rm CH}$) leads almost exclusively to linear HCOOH which further decomposes into OH+HCO. Although the barrier to form dioxirane is only 21.4 kcal/mol the reaction probability to form dioxirane is two orders of magnitude lower if the CH-stretch mode is excited. Following the dioxirane-formation pathway is facile, however, if in addition the COO-bend vibration is excited with energies equivalent to $\sim (2 \nu_{\rm CH} + 4 \nu_{\rm COO})$ or $\sim (3 \nu_{\rm CH} + \nu_{\rm COO})$. For OH-formation in the atmosphere the pathway through linear HCOOH is probably most relevant because the alternative pathways (through dioxirane or formic acid) involve several intermediates that can de-excite through collisions, relax {\it via} Intramolecular vibrational energy redistribution (IVR), or pass through very loose and vulnerable transition states (formic acid). This work demonstrates how, by selectively exciting particular vibrational modes, it is possible to dial into desired reaction channels with a high degree of specificity for a process relevant to atmospheric chemistry.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}

